Surface Quasigeostrophic Turbulence in Variable Stratification

Numerical and observational evidence indicates that, in regions where mixed-layer instability is active, the surface geostrophic velocity is largely induced by surface buoyancy anomalies. Yet, in these regions, the observed surface kinetic energy spectrum is steeper than predicted by uniformly stratified surface quasigeostrophic theory. By generalizing surface quasigeostrophic theory to account for variable stratification, we show that surface buoyancy anomalies can generate a variety of dynamical regimes depending on the stratification's vertical structure. Buoyancy anomalies generate longer range velocity fields over decreasing stratification and shorter range velocity fields over increasing stratification. As a result, the surface kinetic energy spectrum is steeper over decreasing stratification than over increasing stratification. An exception occurs if the near surface stratification is much larger than the deep ocean stratification. In this case, we find an extremely local turbulent regime with surface buoyancy homogenization and a steep surface kinetic energy spectrum, similar to equivalent barotropic turbulence. By applying the variable stratification theory to the wintertime North Atlantic, and assuming that mixed-layer instability acts as a narrowband small-scale surface buoyancy forcing, we obtain a predicted surface kinetic energy spectrum between $k^{-4/3}$ and $k^{-7/3}$, which is consistent with the observed wintertime $k^{-2}$ spectrum. We conclude by suggesting a method of measuring the buoyancy frequency's vertical structure using satellite observations.

==> SQG turbulence in variable stratification (revision II)/PersonalDef.tex <==



% Personal Defintions
\newcommand{\abs}[1]{\left \lvert #1 \right\rvert} % for absolute value
\newcommand{\norm}[1]{\lVert #1 \rVert} % for absolute value
\newcommand{\avg}[1]{\left< #1 \right>} % for average
\newcommand{\inner}[2]{\left< #1, #2 \right>} % for average


\let\foo=\d % rename builtin command \d{} to \underdot{}
\renewcommand{\vec}[1]{\boldsymbol{#1}  } % for vectors
%\newcommand{\p}{\partial}
\newcommand{\lb}{\left}
\newcommand{\rb}{\right}
\renewcommand{\d}[2]{\frac{\mathrm{d} #1}{\mathrm{d} #2}} % for derivatives
\newcommand{\dd}[2]{\frac{\mathrm{d}^2 #1}{\mathrm{d} #2^2}} % for double derivatives
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}} % for partial derivatives
\newcommand{\pdt}[2]{\frac{\partial^2 #1}{\partial #2^2}} % for double partial derivatives
\newcommand{\pdd}[3]{\frac{\partial^2 #1}{\partial #2 \partial#3}} % for double partial derivatives
\newcommand{\pdc}[3]{\left( \frac{\partial #1}{\partial #2}
	\right)_{#3}} % for thermodynamic partial derivatives
\newcommand{\fd}[2]{\frac{\delta #1}{\delta #2}} % for functional derivatives
\newcommand{\fdd}[2]{\frac{\delta^2 #1}{\delta #2^2}} % for second partial derivatives
\newcommand{\grad}[1]{\vec{\nabla} #1} % for gradient
\let\divsymb=\div % rename builtin command \div to \divsymb
\renewcommand{\div}[1]{ \vec{\nabla} \cdot #1} % for divergence
\newcommand{\divh}[1]{ \vec{\nabla}_z \cdot #1} % for divergence
\newcommand{\lap}{\nabla^2} % for laplacian 
\newcommand{\laptwo}{\nabla^4} % for laplacian squared 
\newcommand{\lapz}{\nabla_z^2} % for laplacian 
\newcommand{\curl}[1]{\vec{\nabla} \cross #1} % for curl
\newcommand{\curlh}[1]{\vec{\nabla}_z \cross #1} % for curl
\newcommand{\D}[2]{\frac{D #1}{D #2}} % for Lagrangian derivatives
\newcommand{\cross}{\wedge}  % \cross for cross product
\renewcommand{\bar}{\overline} % \bar for writing an overline
\newcommand{\unit}[1]{\hat{\vec{#1}}}
\newcommand{\dV}{d^3 \vec x \ }
\newcommand{\dVt}{d^2 \vec x \ }
\newcommand{\dVn}[1]{d^#1 \vec x \ }
\newcommand{\dVa}{ d^3\vec a \ }



\newcommand{\reff}[1]{ \left(\ref{#1}\right)} % for divergence

%\newcommand{\ov}[1]{\overline{#1} }
\newcommand{\ov}[1]{{#1}^\ast }

\newcommand{\wh}[1]{\widehat{#1} }

